DESCGEN: A Distantly Supervised Dataset for Generating Abstractive Entity Descriptions

Short textual descriptions of entities provide summaries of their key attributes and have been shown to be useful sources of background knowledge for tasks such as entity linking and question answering. However, generating entity descriptions, especially for new and long-tail entities, can be challenging since relevant information is often scattered across multiple sources with varied content and style. We introduce DESCGEN: given mentions spread over multiple documents, the goal is to generate an entity summary description. DESCGEN consists of 37K entity descriptions from Wikipedia and Fandom, each paired with nine evidence documents on average. The documents were collected using a combination of entity linking and hyperlinks to the Wikipedia and Fandom entity pages, which together provide high-quality distant supervision. The resulting summaries are more abstractive than those found in existing datasets and provide a better proxy for the challenge of describing new and emerging entities. We also propose a two-stage extract-then-generate baseline and show that there exists a large gap (19.9% in ROUGE-L) between state-of-the-art models and human performance, suggesting that the data will support significant future work.

==> sections/backup/introduction.tex <==
\section{Introduction}
% 1. entity knowledge is crucial for solving many tasks ....
% 2. recent work shows that it can be provided in textual form alone (entity knowledge comes from  textual description.)
% 3. curating knowledge is expensive..
% 4. propose the task
% 5. update new emerging entity

Entity knowledge has been shown to play an important role in various applications including language modeling~\cite{peters2019knowledge}, open-domain question answering~\cite{xu-etal-2016-question}, and dialogue generation~\cite{qin-etal-2019-entity}.
Recent studies suggest that essential entity knowledge is greatly captured by textual descriptions~\cite{chen2019enteval}, which can be incorporated to improve downstream tasks~\cite{nie2018mention, logeswaran2019zero}.
However, manually curating entity descriptions is labor-intensive and cannot keep pace with the emergence of new entities. We introduce a new task and dataset \ourdataset~for automatically generating entity descriptions from relevant documents and mentions. For example, in Figure \ref{tbl:example}, machines are required to generate a description of \textit{Carl Menger}, given multiple documents mentioning him.  

\input{tables/example.tex}

In support of the \ourdataset~task, we present a dataset consisting of 37k entity descriptions extracted from Wikipedia and Fandom. Using Fandom allows us to capture the key challenge of generating descriptions for out-of-Wikipedia emerging entities.
% We obtain source documents of entities by distant supervision method. 
To obtain source documents of the entities, we collect web documents and news articles where entity mentions are linked using web hyperlinks or an entity linker.
Our dataset is \emph{distantly supervised} in that these heuristically collected documents are not guaranteed to contain all the facts required to generate the description.
We build a human-annotated subset of 1,000 examples for more reliable assessment.

% Our task is related to multi-document summarization, but it poses additional challenges. Multi-document summarization focuses on creating a summary from a thematically-related document collection (....).  However, source documents of an entity in our task usually belong to various topics and only marginally mention the entity, which makes more difficult to find relevant information. For instance, the document 1 and 2 mentioning \textit{Carl Menger} in Figure~\ref{tbl:example} discuss topics on bitcoins and the Austrian School of Economics. 
% Additionally, 
% in contrast to generic summarization, \ourdataset~requires models to identify texts that are correlated with biographical information about the entity.


% \ourdataset~is more challenging than multi-document summarization which aims to create a summary from thematically-related document collection~\ref{zopf2016next}. For example, the Multi-News 

% \ourdataset~ is related to multi-document summarization, but it poses additional challenges. Multi-document summarization aims to create a summary from document clusters on the same topic~\ref{zopf2016next}. For example ... However, source documents of an entity in our task usually belong to various topics and only marginally mention the entity, which makes more difficult to find relevant information. 
% For instance, the document 1 and 2 mentioning \textit{Carl Menger} in Figure~\ref{tbl:example} discuss topics on bitcoins and the Austrian School of Economics. 
% Additionally,  
The entity-centric nature of \ourdataset~poses a key challenge of identifying relavant information scattered in heterogeneous source documents and unifying it into a well-organized description covering essential aspects of the entity. Unlike multi-document summarization that makes the assumption that a set of documents to be summarized are written on the same topic~\cite{zopf2016next}, \ourdataset~only assumes that source documents mention the entity. Therefore, documents for generating an description 
can belong to various topics as well as text genres, including news, blog posts and scientific articles.
% and only marginally mention the entity. 
For instance, the document 1 and 2 mentioning \textit{Carl Menger} in Figure~\ref{tbl:example} discuss topics on bitcoins and the Austrian School of Economics. The diversity in documents topics and text genres make more difficult to find entity-relevant information.   
% \ourdataset~ makes weak assumption that documents for generating an description can belong to various topics as well as text genres, and only marginally mention the entity. aims to generate entity descriptions from topic unrelated documents 
% Our task is more challenging than multi-document summarization because 
% in multi-document summarization, a set of documents to be summarized is assumed to be on the same topic. 
% For example, the MultiNews dataset () consists of 56,000 clusters focusing on 
% However, source 

% which aims to creating a summary from document clusters on the same topic~\ref{zopf2016next}. 
% In multi-document summarization, a set of documents to be summarized is assumed to be on the same topic.

% Existing corpora for multi-document summarization such as ... and ... exclusively focus on 
% For example, the MultiNews dataset consists of xxx clusters 


% Despite the fact that \ourdataset~ is similar in set up to multi-document summarization, it poses more of a challenge. 
% With the goal of creating a summary from document clusters on the same topic~\ref{zopf2016next}, existing multi-document summarization corpora focuses on 

% Multi-document summarization aims to create a summary from document clusters on the same topic~\ref{zopf2016next}. For example, the MultiNews dataset consists of xxx clusters 


% The key challenge of \ourdataset~ is how to identify information in and fuse them into 

% 1. relate to MDS, more challenges
% - same topic, different topic, example
% - 


% % \todo{Wikipedia quality low + description can benefit various tasks} 
% Entity descriptions, including lead sections of Wikipedia and actor biographies from IMDB, provide encyclopedic overviews of entity. 
% They are important for various applications such as entity linking~\cite{nie2018mention, logeswaran-etal-2019-zero}, knowledge base completion~\cite{pezeshkpour-etal-2018-embedding, shi2018open} and open-domain question answering~\cite{sun2015open, xu-etal-2016-question}. 
% Despite the fact that Wikipedia has over 6 million English articles covering entities on diverse topics, its growth cannot keep pace with the emergence of entities. It has been aware that Wikipedia, manually curated by knowledgeable editors, is overwhelmingly incomplete on long-tail and newly emerging entities~\cite{akasaki2019early}. To address this challenge, we propose a new task \ourdataset~that aims to generate an entity description from automatically aggregated documents mentioning the entity. For example, in Figure \ref{tbl:example}, machines are required to generate a biography of \textit{Carl Menger}, given multiple documents mentioning him. 
% \begin{figure}[h]
% \includegraphics[width=1\linewidth]{pic/test.pdf}
% \caption{
% An example entity description of Bowser and its source documents.
% }
% \label{fig:example}
% \end{figure}
% and covers most significant knowledge in its description.
% entity descriptions tend to contain biographical information, which requires models to characterize texts that are essential in biography domain.


% To ensure that our task is solvable by human, we crowdsourced a human-annotated subset of 1,000 examples. 
% For evaluation, we report results on human-annotated subset of 1,000 examples. 

% (Our work is most related to previous work on generating Wikipedia summaries~\cite{liu2018generating}. They build a large-scale multi-document summarization dataset by collecting documents primarily from cited sources (75\% documents) make significantly more extractive than our dataset (see section ...), which contains carefully curated encyclopedic knowledge about the entity. 
% In contrast, \ourdataset~exploits web texts and news, which realistically resemble use cases of generating descriptions for emerging entities in their early-stage appearance.
% They also evaluate on weakly-supervised test set, which makes difficult to measure performance gain.
% Our carefully curated human test sets shows drop is high
% In addition, their evaluation is conducted with distant supervision. However, a Wikipedia summary is not guaranteed to be well supported by citations.
% We address this shortcoming by evaluating on human annotated datasets, which makes automatic evaluation in this setting more reliable.)


Our work is most related to previous work on generating Wikipedia summaries~\cite{liu2018generating}. Their source documents for summarization primarily come from high-quality articles cited in the Wikipedia pages (75\% of all documents). 
which makes their dataset more extractive than \ourdataset~(see section~\ref{extractive}). 
In contrast, we collect our source documents automatically from web texts and news because it resembles use cases of generating descriptions for emerging entities when hand-picked citation sources are not available.
In addition, their evaluation is conducted only on distantly supervised test data. However, our experiments demonstrate that the ranking list of models on distant supervised test set and human-annotated test set are different (see Table~\ref{result}), indicating that the carefully curated test data is necessary.
% a significant gap exists between distant supervision evaluation and 
% aims to generate entity descriptions from web texts and news, which
% In contrast, we
% As opposed to carefully curated citations, web texts and news articles in our task are closer to 
% This leads to our motivation of generating entity descriptions for emerging and long-tail entities.
% In addition, their evaluation is conducted with distant supervision only. 
% previous work on generating Wikipedia summaries (....). They collected 
% whereas we use news articles and we
% 1. related to Wikisum
% - motivation is different --> citation source
% we use news articles (primary sources) and web text --> emerging entity
% - their evaluation is conducted with automatically 



% no careful dev and test sets to carefully measure the performance
% In addition, they assume 
% - task is able to do by human
% - dataset challenge

With a new task definition and its dataset, we propose a two-stage method
that first extracts salient sentences relevant to the entity and then abstract them into a description. We test a range of models to establish baseline results with both automatic and human evaluation. The best model based on BART~\cite{lewis-etal-2020-bart} achieves 28.2\% in the ROUGE-L F measure with a significant gap compared to the human performance 48.1\%, suggesting there was great room for future improvement. We summarize our contributions as follows:  
\begin{itemize}
    \item We propose a new task \ourdataset~that aims to automate the process of generating entity descriptions. We construct a dataset for this task, which contains over 37K pairs of entity descriptions and their associated documents, along with a human-annotated subset of 1,000 pairs.
    \item We conduct an extensive analysis of properties of the dataset and identify challenges in solving \ourdataset.
    \item We present a two-stage method and benchmark various models on our dataset, aiming to facilitate future work on this dataset.
    % demonstrating the difficulty of the task.
\end{itemize}




% Such applications often require knowledge of long-tail and emerging entities...
% For example, entity linking aims to link mentions in a document to its corresponding entries in a knowledge base such as Wikipedia. However, due to the incompleteness of Wikipedia, emerging entities cannot be linked.   
% Despite the fact that Wikipedia has over 6 million English articles covering entities on diverse topics, 
% However, the growth of Wikipedia, hindered by the availability of knowledgeable editors, falls behind the emergence of entities. It has been aware that Wikipedia is overwhelmingly incomplete on long-tail and newly emerging entities~\cite{akasaki2019early}. 

% To automate the process of curating entity descriptions, we propose a new task



% cannot keep pace with the emergence of entities. 
% popular entities are covered in great details, but there are long-tail and newly emerging entities with little or no descriptions. Therefore, it 

% and therefore cannot keep pace with the emergence of entities. 


% A Knowledge Base (KB) can be viewed as an encyclopedia about entities. It contains definitional and relation data for entities. However, KBs such as Wikipedia are far from complete: newly emerging entities are added to them every day. 
% We refer to such entities as out-of-KB entities or emerging entities. Although previous works (TAC KBP) introduce the task of linking out-of-KB entities to NIL and do NIL clustering, they do not carefully model their representation. 
% After an emerging entity is observed sufficiently often, it is important to write its description that is understandable to users. Such descriptions are fundamental for extending KBs and linking further texts to this entity. 

% \todo{motivation + introduce the task} \\
% Curating descriptions by hand is a labor-intensive work. It requires editors to read through a large number of source documents about entities, identify relevant information and write a concise and coherent description. To automate this process, we introduce a new task: given multiple source documents that mention the entity, the aim is to automatically generate its description. Figure \ref{fig:example} shows an example of source documents about the Mario character Bowser and its generated description.



% \todo{different from multi-document summarizaion: docs differ topics + } \\
% Our proposed task can be approached as multi-document summarization --- task of producing informative and brief summaries from clusters of thematically related documents. Nonetheless, it poses two additional challenges. First, multi-document summarization makes the assumption that input documents are written about the same topic.  .... In addition, the input documents tend to be noisy and irrelevant to the generated description/summary ....
% 1. not rare entities (Wikipedia summaries generation)
% 2. extraction of information from multiple texts written about the same topic.
% 3. 

% \todo{introduce our dataset and explain how it is different from previous datasets} \\
% Prior works on generating Wikipedia summary from referenced documents tap a little into description generation. 

% \todo{baseline model and summarize our contribution} \\
% unique entities with source documents extracted from the web pages and entity descriptions from Wikipedia and Fandom\footnote{https://www.fandom.com}. 

% Compared to 
% \input{tables/example}


% challenges? This requires the ability to link indi

% In summary, our contribution are as follows


% motivation
% task
% related to .. task
% dataset + challenge
% baseline model
% contribution

% compared with Liu, why not use reference doucments
% \newpage

==> tables/gram.tex <==
\begin{table}[!tb]
\centering
\small
{
\setlength{\tabcolsep}{0.3em}
    \begin{tabular}{l|c|c|c|c}
    \toprule[0.7pt]
    \textbf{n-grams}   & \textbf{unigram}  & \textbf{bigrams}  & \textbf{trigrams} & \textbf{4-grams}   \\ \hline
    Ours  & 80.20  & 43.43  & 19.21 & 10.80\\    
    Multi-News & 82.24 & 42.9 & 24.29 & 17.70 \\
    % DUC03+04 & 72.26 & 38.82 & 9.39 & 3.82\\
    CNN/DailyMail & 80.50 & 43.12 & 25.59 & 17.17 \\

    
    
    
    \bottomrule[0.7pt]
    \end{tabular} 
}
\caption{N-gram recall (\%) for summarization datasets.}
\label{tbl:recall}
\end{table}


==> tables/result.tex <==
\begin{table*}[htbp]
\small
  \begin{center}
  
    \begin{tabular}{c|c|ccc|ccc|ccc|ccc} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
    \toprule[0.7pt]
      \multirow{3}{*}{\textbf{Extract.}} & \multirow{3}{*}{\textbf{Abstract.}} & \multicolumn{6}{c|}{Distant supervision} &  \multicolumn{6}{c}{Verified} \\

      & & \multicolumn{3}{c|}{Dev} &  \multicolumn{3}{c|}{Test} & \multicolumn{3}{c|}{Dev} &  \multicolumn{3}{c}{Test} \\
      & & \texttt{R-1} & \texttt{R-2} & \texttt{R-L} & \texttt{R-1} & \texttt{R-2} & \texttt{R-L} & \texttt{R-1} & \texttt{R-2} & \texttt{R-L} & \texttt{R-1} & \texttt{R-2} & \texttt{R-L} \\
      
      \hline
      \multirow{4}{*}{Trivial}  & BART & 24.5 & 11.3 & 22.1 & 23.4 & 10.7 & 23.8 & 27.2 & 14.2 & 26.4 & 27.1 & 15.9 & 26.6\\
      & T5-Base & 21.7 & 9.3 & 20.6 & 21.1 & 10.5 & 21.1 & 25.1 & 12.8 & 24.7 & 24.9 & 13.2 & 23.7 \\
      & T5-Large & 23.9 & 12.7 & 23.4 & 24.2 & 11.1 & 23.5 & 27.7 & 15.9 & 27.2 & 26.9 & 15.6 & 27.3 \\
      & MARGE & 23.2 & 10.6 & 21.8 & 23.0 & 10.2 & 22.1 & 26.4 & 13.9 & 25.8 & 26.2 & 14.0 & 25.8 \\

        \hline
      \multirow{4}{*}{BERT} & BART & \textbf{26.9} & 13.9 & \textbf{27.6} & \textbf{26.3} & 13.2 & \textbf{26.6} & \textbf{28.9} & \textbf{16.9} &  27.3 & 26.7 & \textbf{16.4} & \textbf{28.2} \\
    & T5-Base & 23.4 & 10.1 & 23.9 & 23.0 & 11.6 & 24.4 & 24.9 & 11.7 & 24.1 & 25.0 & 12.2 & 24.8  \\
    & T5-Large & 26.8 & \textbf{15.1} & 27.4 &   25.4 & \textbf{14.8} & 25.9 & 27.1 & 16.6 & \textbf{27.5} & \textbf{27.3} & 16.1 & 27.3 \\
      & MARGE & 25.1 & 13.8 & 26.2 & 24.9 & 11.9 & 25.0 & 26.7 & 15.7 & 25.9 & 26.3 & 14.8 & 25.8 \\
        \hline
    \multicolumn{2}{c|}{Human Performance}  & 34.8 & 18.3 & 33.5 &  35.3 & 18.5 & 34.4 & 45.2 & 36.7 & 48.7 & 45.3 & 35.4 & 48.1\\
      
      
         \bottomrule[0.7pt]

    \end{tabular}
      \caption{Experimental results of different baselines evaluated on distantly supervised and verified dev/test sets.}
    \label{result}
  \end{center}
\end{table*}

==> tables/wikisum.tex <==
\begin{table}[!tb]
\centering
\small
{
\setlength{\tabcolsep}{0.3em}
    \begin{tabular}{lcc}
    \toprule[0.7pt]
    \textbf{Training corpus}   & \textbf{Testing} &  \textbf{ROUGE-L}  \\ \hline
    WikiSum & Wikipedia & 25.3 \\
    WikiSum & WikiSum & 34.7 \\
    \ourdataset &  Wikipedia & 28.4 \\
    \ourdataset & WikiSum & 31.5 \\
    WikiSum & Fandom & 22.8 \\
    \ourdataset &  Fandom & 27.5 \\
    
    \bottomrule[0.7pt]
    \end{tabular} 
}
\caption{ROUGE-L scores for BERT+BART trained on WikiSum but tested on our verified test set.}
\label{tbl:type}
\end{table}

